StyleMorpheus: A Style-Based 3D-Aware Morphable Face Model

For 3D face modeling, the recently developed 3D-aware neural rendering methods are able to render photorealistic face images with arbitrary viewing directions. The training of the parametric controllable 3D-aware face models, however, still relies on a large-scale dataset that is lab-collected. To address this issue, this paper introduces "StyleMorpheus", the first style-based neural 3D Morphable Face Model (3DMM) that is trained on in-the-wild images. It inherits 3DMM's disentangled controllability (over face identity, expression, and appearance) but without the need for accurately reconstructed explicit 3D shapes. StyleMorpheus employs an auto-encoder structure. The encoder aims at learning a representative disentangled parametric code space and the decoder improves the disentanglement using shape and appearance-related style codes in the different sub-modules of the network. Furthermore, we fine-tune the decoder through style-based generative adversarial learning to achieve photorealistic 3D rendering quality. The proposed style-based design enables StyleMorpheus to achieve state-of-the-art 3D-aware face reconstruction results, while also allowing disentangled control of the reconstructed face. Our model achieves real-time rendering speed, allowing its use in virtual reality applications. We also demonstrate the capability of the proposed style-based design in face editing applications such as style mixing and color editing. Project homepage: https://github.com/ubc-3d-vision-lab/StyleMorpheus.

==> literature_table.tex <==
\begin{table}[ht]
    %\small
    \centering
    \caption{A brief comparison of existing 3D-aware face models.}
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|} \hline
         \textbf{Method} & \textbf{Year} &
         \textbf{\makecell{3DMM\\Used}} &
         \textbf{\makecell{Disentangled\\Control}} &
         \textbf{\makecell{Include\\Hair}} & 
         \textbf{\makecell{3D Rep.}} & 
         \textbf{\makecell{Code\\Dim.}} & 
         \textbf{\makecell{Real-\\time}} &
         \textbf{\makecell{Reconstruction\\Approach}} &
         \textbf{\makecell{Training\\Dataset(s)}} 
         \\\hline

        StyleNeRF \cite{gu2021stylenerf} & 2021 & \xmark & P & \cmark & \makecell{NeRF} & 512 & \xmark & GAN Inversion & FFHQ \cite{karras2019style}
        \\\hline
        CIPS-3D \cite{zhou2021cips} & 2021 & \xmark & P & \cmark & \makecell{NeRF} & 768 & \xmark & GAN Inversion & FFHQ
        \\\hline
        EG3D \cite{chan2022efficient} & 2022 & \xmark & P & \cmark & \makecell{NeRF} & 512 & \cmark & GAN Inversion & FFHQ 
        \\\hline
        FENeRF \cite{sun2022fenerf} & 2022 & \xmark & P & \cmark & \makecell{NeRF} & 512 & \xmark & GAN Inversion & \makecell{CelebA-HQ \cite{celebahq},\\FFHQ}
        \\\hline
        MoFaNeRF \cite{zhuang2022mofanerf} & 2022 & \xmark & S,E,T & \xmark & \makecell{NeRF} & 336 & \xmark & Fitting & \makecell{FaceScape \cite{yang2020facescape},\\HeadSpace \cite{dai2020statistical}} 
        \\\hline
        CGoF \cite{sun2022controllable}  & 2022 & BFM \cite{blanz1999morphable} & S,E,T & \cmark & \makecell{Hybrid} & 411 & - & \makecell{3DMM Fitting\\+ GAN Inversion} & \makecell{CelebA \cite{liu2015faceattributes},\\FFHQ} 
        \\\hline
        HeadNeRF \cite{hong2022headnerf} & 2022 & \makecell{NL3DMM\\ \cite{tran2018nonlinear}} & S,E,T,L & \cmark & \makecell{NeRF} & 306 & \cmark & \makecell{3DMM Fitting\\+ Code Fine-tuning} & \makecell{FaceScape,\\FaceSEIP \cite{hong2022headnerf},\\FFHQ} 
        \\\hline
        OmniAvatar \cite{xu2023omniavatar} & 2023 & FLAME \cite{FLAME:SiggraphAsia2017} & S,E,T & \cmark & \makecell{Hybrid} & 718 & - & \makecell{3DMM Fitting\\+ GAN Inversion} & \makecell{FLAME Meshes,\\FFHQ} 
        \\\hline
        Next3D \cite{sun2023next3d} & 2023 & FLAME & S,E,T & \cmark & \makecell{Hybrid} & 671 & \xmark & \makecell{3DMM Fitting\\+ GAN Inversion} & FFHQ
        \\\hline
        OTAvatar \cite{ma2023otavatar} & 2023 & BFM & \cmark (S,E,T) & \cmark & \makecell{NeRF} & 576 & \cmark & \makecell{3DMM Fitting\\+ GAN Inversion} & HDTF \cite{zhang2021flow}
        \\\hline
        CIPS-3D++ \cite{zhou2023cips} & 2023 & \xmark & P & \cmark & \makecell{NeRF} & 768 & \xmark & GAN Inversion & FFHQ
        \\\hline
        3DMM-RF \cite{galanakis20233dmm} & 2023 & BFM & S,E,T,L  & \xmark & \makecell{NeRF} & 540 & - & GAN Inversion & Synthetic Data
        \\\hline
        Ours & 2023 & NL3DMM & S,E,T,L & \cmark & \makecell{NeRF} & 306 & \cmark & \makecell{Encoder\\+ Code Fine-tuning} & FFHQ   
        \\\hline

        \multicolumn{9}{l}{P: camera pose; S: shape; E: expression; T: texture; L: lighting.}\\
        \multicolumn{9}{l}{- indicates the information is not available.}\\

    \end{tabular}
    \label{tab:literature}
\end{table}



